Synthetic Object Compositions for Scalable and Accurate Learning in Detection, Segmentation, and Grounding

Visual grouping -- operationalized through tasks such as instance segmentation, visual grounding, and object detection -- enables applications ranging from robotic perception to photo editing. These fundamental problems in computer vision are powered by large-scale, painstakingly annotated datasets. Despite their impact, these datasets are costly to build, biased in coverage, and difficult to scale. Synthetic datasets offer a promising alternative but struggle with flexibility, accuracy, and compositional diversity. We introduce Synthetic Object Compositions (SOC), an accurate and scalable data synthesis pipeline via a novel object-centric composition strategy. It composes high-quality synthetic object segments into new images using 3D geometric layout augmentation and camera configuration augmentation with generative harmonization and mask-area-weighted blending, yielding accurate and diverse masks, boxes, and referring expressions. Models trained on just 100K of our synthetic images outperform those trained on larger real datasets (GRIT 20M, V3Det 200K) and synthetic pipelines (Copy-Paste, X-Paste, SynGround, SegGen) by +24-36% -- achieving +10.9 AP on LVIS and +8.4 NAcc on gRefCOCO. Beyond the general open-vocabulary setup, SOC also enables controllable dataset construction for different use cases and boosts performance in both low-data and closed-vocabulary scenarios. Augmenting LVIS and COCO with synthetic object segments delivers strong performance across different real-data scales and yields even greater improvements under extremely limited real-data conditions, including +6.59 AP on a 1% COCO data setup. Furthermore, this controllability enables targeted data generation for intra-class referring, a diagnostic grounding task we propose that requires fine-grained attribute discrimination.

==> tables/grounding_dino_overall.tex <==
\begin{table}[htbp]
  \centering
  \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{lccccccccc}
    \toprule
    \textbf{Metric} & \textbf{\texttt{O365+GoldG}} & \textbf{\texttt{O365+GoldG+GRIT}} & \textbf{\texttt{O365+GoldG+V3Det}} & \textbf{\texttt{O365+GoldG+GRIT+V3Det}} & \textbf{\texttt{1.3k\_category}} & \textbf{\texttt{1.3k\_and\_40k\_category}} & \textbf{\texttt{1.3k\_and\_40k\_mixup}} & \textbf{\texttt{ovd\_50k\_mixup\_relightening\_4\_21\_open\_finetune}} & \textbf{\texttt{ovd\_50k\_mixup\_relightening\_4\_21\_open\_stage2\_finetune}} \\
    \midrule
    \texttt{coco/bbox\_mAP} & 50.4 & 50.5 & 50.6 & 50.4 & 48.7 & 48.0 & 47.2 & 48.4 & 48.5 \\
    \bottomrule
    \end{tabular}
  \end{adjustbox}
  \caption{Results for \texttt{grounding\_dino\_swin-t\_pretrain\_coco\_eval}.}
  \label{tab:grounding_dino_swin_t_pretrain_coco_eval}
\end{table}

\begin{table}[htbp]
  \centering
  \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{lccccccccc}
    \toprule
    \textbf{Metric} & \textbf{\texttt{O365+GoldG}} & \textbf{\texttt{O365+GoldG+GRIT}} & \textbf{\texttt{O365+GoldG+V3Det}} & \textbf{\texttt{O365+GoldG+GRIT+V3Det}} & \textbf{\texttt{1.3k\_category}} & \textbf{\texttt{1.3k\_and\_40k\_category}} & \textbf{\texttt{1.3k\_and\_40k\_mixup}} & \textbf{\texttt{ovd\_50k\_mixup\_relightening\_4\_21\_open\_finetune}} & \textbf{\texttt{ovd\_50k\_mixup\_relightening\_4\_21\_open\_stage2\_finetune}} \\
    \midrule
    \texttt{lvis\_fixed\_ap/AP} & 35.7 & 36.5 & 40.5 & 41.4 & 39.3 & 38.8 & 38.8 & 39.5 & 40.0 \\
    \texttt{lvis\_fixed\_ap/APc} & 30.2 & 32.4 & 36.0 & 37.4 & 37.3 & 36.2 & 37.3 & 37.9 & 39.2 \\
    \texttt{lvis\_fixed\_ap/APf} & 42.0 & 41.8 & 45.9 & 46.2 & 42.4 & 41.9 & 41.1 & 41.6 & 41.5 \\
    \texttt{lvis\_fixed\_ap/APr} & 28.1 & 26.6 & 33.0 & 34.2 & 32.0 & 34.8 & 33.0 & 36.3 & 35.9 \\
    \bottomrule
    \end{tabular}
  \end{adjustbox}
  \caption{Results for \texttt{grounding\_dino\_swin-t\_pretrain\_zeroshot\_mini-lvis}.}
  \label{tab:grounding_dino_swin_t_pretrain_zeroshot_mini_lvis}
\end{table}

\begin{table}[htbp]
  \centering
  \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{lcccccccc}
    \toprule
    \textbf{Metric} & \textbf{\texttt{O365+GoldG}} & \textbf{\texttt{O365+GoldG+GRIT}} & \textbf{\texttt{O365+GoldG+V3Det}} & \textbf{\texttt{O365+GoldG+GRIT+V3Det}} & \textbf{\texttt{1.3k\_category}} & \textbf{\texttt{1.3k\_and\_40k\_category}} & \textbf{\texttt{1.3k\_and\_40k\_mixup}} & \textbf{\texttt{ovd\_50k\_mixup\_relightening\_4\_21\_open\_stage2\_finetune}} \\
    \midrule
    \texttt{lvis\_fixed\_ap/AP} & 20.1 & 27.1 & 30.6 & 31.9 & 30.7 & 30.8 & 30.2 & 30.2 \\
    \texttt{lvis\_fixed\_ap/APc} & 15.3 & 22.6 & 25.5 & 27.6 & 27.4 & 27.4 & 27.3 & 27.4 \\
    \texttt{lvis\_fixed\_ap/APf} & 29.9 & 36.4 & 40.2 & 40.5 & 36.9 & 36.2 & 35.4 & 36.0 \\
    \texttt{lvis\_fixed\_ap/APr} & 10.1 & 17.3 & 21.5 & 23.6 & 24.9 & 27.0 & 25.7 & 24.2 \\
    \bottomrule
    \end{tabular}
  \end{adjustbox}
  \caption{Results for \texttt{grounding\_dino\_swin-t\_pretrain\_zeroshot\_lvis}.}
  \label{tab:grounding_dino_swin_t_pretrain_zeroshot_lvis}
\end{table}

\begin{table}[htbp]
  \centering
  \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{lccccccccc}
    \toprule
    \textbf{Metric} & \textbf{\texttt{O365+GoldG}} & \textbf{\texttt{O365+GoldG+GRIT}} & \textbf{\texttt{O365+GoldG+V3Det}} & \textbf{\texttt{O365+GoldG+GRIT+V3Det}} & \textbf{\texttt{1.3k\_category}} & \textbf{\texttt{1.3k\_and\_40k\_category}} & \textbf{\texttt{1.3k\_and\_40k\_mixup}} & \textbf{\texttt{ovd\_50k\_mixup\_relightening\_4\_21\_open\_finetune}} & \textbf{\texttt{ovd\_50k\_mixup\_relightening\_4\_21\_open\_stage2\_finetune}} \\
    \midrule
    \texttt{AerialMaritimeDrone\_large/coco/bbox\_mAP} & 13.3 & 15.5 & 17.7 & 15.1 & 13.5 & \textbf{16.5} & 15.0 & 13.6 & 16.1 \\
    \texttt{AerialMaritimeDrone\_tiled/coco/bbox\_mAP} & 17.0 & 22.5 & 18.4 & 20.6 & 14.0 & 17.4 & \textbf{17.5} & 15.2 & 16.7 \\
    \texttt{AmericanSignLanguageLetters/coco/bbox\_mAP} & 1.6 & 2.0 & 1.1 & 0.7 & 2.2 & 1.4 & 1.3 & 1.1 & 2.2 \\
    \texttt{Aquarium/coco/bbox\_mAP} & 25.2 & 26.1 & 26.6 & 28.3 & \textbf{26.1} & 24.4 & 25.8 & 23.9 & 25.9 \\
    \texttt{BCCD/coco/bbox\_mAP} & 6.9 & 11.8 & 8.3 & 7.7 & 15.6 & 10.0 & \textbf{17.9} & 12.3 & 16.4 \\
    \texttt{ChessPieces/coco/bbox\_mAP} & 0.0 & 0.0 & 0.0 & 0.0 & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & 0.0 & 0.0 \\
    \texttt{CottontailRabbits/coco/bbox\_mAP} & 77.1 & 81.0 & 77.8 & 78.6 & \textbf{79.4} & 78.8 & 78.1 & 78.3 & 77.5 \\
    \texttt{DroneControl/coco/bbox\_mAP} & 4.7 & 9.7 & 8.8 & 7.4 & 4.4 & 5.6 & 5.5 & 5.0 & 4.5 \\
    \texttt{EgoHands\_generic/coco/bbox\_mAP} & 52.7 & 53.7 & 50.6 & 51.9 & 49.5 & 47.3 & \textbf{50.7} & 48.6 & 52.1 \\
    \texttt{EgoHands\_specific/coco/bbox\_mAP} & 0.1 & 0.5 & 0.7 & 0.3 & 0.2 & 0.0 & 0.7 & 0.2 & 1.9 \\
    \texttt{HardHatWorkers/coco/bbox\_mAP} & 4.8 & 7.0 & 7.0 & 10.8 & 4.5 & 6.6 & 4.6 & 4.8 & 6.1 \\
    \texttt{MaskWearing/coco/bbox\_mAP} & 0.9 & 0.4 & 1.1 & 0.9 & \textbf{2.5} & 0.9 & 1.0 & 2.1 & 2.2 \\
    \texttt{MountainDewCommercial/coco/bbox\_mAP} & 45.3 & 46.5 & 19.4 & 43.0 & 36.6 & \textbf{50.2} & 32.7 & 27.3 & 48.7 \\
    \texttt{NorthAmericaMushrooms/coco/bbox\_mAP} & 33.1 & 46.2 & 66.9 & 76.7 & 42.7 & 18.1 & \textbf{43.9} & 30.7 & 36.9 \\
    \texttt{OxfordPets\_by\_breed/coco/bbox\_mAP} & 0.2 & 0.4 & 0.6 & 0.4 & \textbf{2.6} & 2.5 & 2.0 & 3.7 & 1.9 \\
    \texttt{OxfordPets\_by\_species/coco/bbox\_mAP} & 1.9 & 1.6 & 2.0 & 1.5 & 1.9 & \textbf{2.3} & 1.7 & 2.0 & 1.5 \\
    \texttt{PKLot/coco/bbox\_mAP} & 0.4 & 0.2 & 0.8 & 0.7 & 0.1 & 0.0 & \textbf{0.2} & 0.2 & 0.3 \\
    \texttt{Packages/coco/bbox\_mAP} & 70.7 & 68.7 & 71.0 & 70.6 & \textbf{76.4} & 72.9 & 71.7 & 73.5 & 75.3 \\
    \texttt{PascalVOC/coco/bbox\_mAP} & 56.5 & 58.0 & 56.6 & 56.6 & \textbf{59.4} & 58.4 & 57.2 & 58.4 & 59.4 \\
    \texttt{Raccoons/coco/bbox\_mAP} & 46.9 & 51.1 & 55.3 & 53.5 & 54.1 & 56.1 & 53.1 & 56.6 & 52.1 \\
    \texttt{ShellfishOpenImages/coco/bbox\_mAP} & 32.1 & 43.7 & 51.9 & 48.8 & 35.1 & \textbf{35.4} & 32.6 & 31.6 & 33.1 \\
    \texttt{ThermalCheetah/coco/bbox\_mAP} & 6.3 & 8.1 & 3.0 & 4.5 & 11.6 & 7.9 & 9.5 & 12.6 & 8.1 \\
    \texttt{UnoCards/coco/bbox\_mAP} & 1.2 & 1.0 & 0.9 & 0.5 & 0.6 & \textbf{1.0} & 0.3 & 0.7 & 0.5 \\
    \texttt{VehiclesOpenImages/coco/bbox\_mAP} & 56.6 & 60.3 & 61.4 & 61.5 & 56.8 & \textbf{57.3} & 56.0 & 55.2 & 58.6 \\
    \texttt{WildfireSmoke/coco/bbox\_mAP} & 10.6 & 15.4 & 4.2 & 12.7 & 11.9 & \textbf{12.3} & 5.4 & 14.3 & 6.1 \\
    \texttt{boggleBoards/coco/bbox\_mAP} & 0.2 & 0.1 & 0.1 & 0.2 & \textbf{0.2} & \textbf{0.2} & 0.1 & 0.1 & 0.1 \\
    \texttt{brackishUnderwater/coco/bbox\_mAP} & 3.3 & 2.1 & 2.5 & 2.5 & 2.8 & 3.6 & 2.6 & 3.0 & 1.9 \\
    \texttt{dice/coco/bbox\_mAP} & 0.2 & 0.5 & 0.1 & 0.1 & 0.3 & \textbf{1.0} & 0.6 & 0.3 & 0.2 \\
    \texttt{openPoetryVision/coco/bbox\_mAP} & 0.1 & 0.0 & 0.0 & 0.0 & \textbf{0.5} & 0.2 & 0.4 & 0.4 & 0.1 \\
    \texttt{pistols/coco/bbox\_mAP} & 58.5 & 70.9 & 67.1 & 72.9 & \textbf{58.4} & 51.8 & 54.4 & 57.4 & 53.9 \\
    \texttt{plantdoc/coco/bbox\_mAP} & 0.5 & 0.7 & 0.8 & 1.1 & 1.2 & 1.2 & \textbf{1.3} & 1.7 & 1.8 \\
    \texttt{pothole/coco/bbox\_mAP} & 13.6 & 21.9 & 7.7 & 16.8 & 10.3 & 9.0 & \textbf{10.5} & 12.0 & 12.2 \\
    \texttt{selfdrivingCar/coco/bbox\_mAP} & 9.1 & 7.6 & 9.4 & 8.3 & 8.1 & 7.9 & \textbf{9.4} & 6.9 & 8.8 \\
    \texttt{thermalDogsAndPeople/coco/bbox\_mAP} & 55.6 & 60.3 & 49.3 & 54.3 & 49.0 & \textbf{54.7} & 49.1 & 56.3 & 53.6 \\
    \texttt{websiteScreenshots/coco/bbox\_mAP} & 2.0 & 1.6 & 1.6 & 1.6 & \textbf{2.1} & 2.0 & \textbf{2.1} & 2.4 & 2.0 \\
    \textbf{Average} & 20.3 & 22.8 & 21.4 & 23.2 & 21.0 & 20.4 & 20.4 & 20.4 & 21.1 \\
    \bottomrule
    \end{tabular}
  \end{adjustbox}
  \caption{Results for \texttt{grounding\_dino\_swin-t\_pretrain\_odinw35}.}
  \label{tab:grounding_dino_swin_t_pretrain_odinw35}
\end{table}

\begin{table}[htbp]
  \centering
  \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{lccccccccc}
    \toprule
    \textbf{Metric} & \textbf{\texttt{O365+GoldG}} & \textbf{\texttt{O365+GoldG+GRIT}} & \textbf{\texttt{O365+GoldG+V3Det}} & \textbf{\texttt{O365+GoldG+GRIT+V3Det}} & \textbf{\texttt{1.3k\_category}} & \textbf{\texttt{1.3k\_and\_40k\_category}} & \textbf{\texttt{1.3k\_and\_40k\_mixup}} & \textbf{\texttt{ovd\_50k\_mixup\_relightening\_4\_21\_open\_finetune}} & \textbf{\texttt{ovd\_50k\_mixup\_relightening\_4\_21\_open\_stage2\_finetune}} \\
    \midrule
    \texttt{grefcoco\_testA/grefcoco/F1\_score} & 26.3 & 26.0 & 25.4 & 26.1 & 25.8 & 25.8 & 25.3 & 24.5 & 26.6 \\
    \texttt{grefcoco\_testA/grefcoco/N\_acc} & 91.2 & 91.2 & 91.2 & 91.2 & 91.2 & 92.5 & 93.8 & 93.0 & 89.0 \\
    \texttt{grefcoco\_testA/grefcoco/T\_acc} & 89.0 & 91.9 & 91.8 & 93.0 & 16.5 & 16.1 & 13.5 & 13.9 & 19.9 \\
    \texttt{grefcoco\_testB/grefcoco/F1\_score} & 31.3 & 30.6 & 30.7 & 30.4 & 30.4 & 30.6 & 30.6 & 29.9 & 31.2 \\
    \texttt{grefcoco\_testB/grefcoco/N\_acc} & 90.9 & 90.9 & 90.9 & 90.9 & 90.9 & 91.6 & 94.5 & 92.0 & 87.2 \\
    \texttt{grefcoco\_testB/grefcoco/T\_acc} & 84.8 & 90.2 & 89.9 & 92.3 & 14.2 & 13.1 & 10.2 & 11.6 & 18.0 \\
    \texttt{grefcoco\_val/grefcoco/F1\_score} & 39.8 & 40.7 & 40.3 & 41.0 & 40.4 & 40.9 & 41.1 & 40.2 & 40.3 \\
    \texttt{grefcoco\_val/grefcoco/N\_acc} & 89.3 & 89.3 & 89.3 & 89.3 & 89.3 & 90.8 & 92.5 & 90.6 & 86.2 \\
    \texttt{grefcoco\_val/grefcoco/T\_acc} & 84.7 & 89.7 & 88.8 & 91.3 & 13.4 & 13.1 & 10.5 & 11.7 & 17.5 \\
    \texttt{refcoco+\_testA/refexp/refcoco+\_precision\@1} & 57.3 & 59.0 & 58.1 & 58.7 & 58.5 & 57.4 & 58.4 & 57.9 & 57.8 \\
    \texttt{refcoco+\_testA/refexp/refcoco+\_precision\@10} & 92.7 & 93.7 & 93.5 & 93.1 & 91.9 & 92.4 & 92.0 & 92.4 & 93.0 \\
    \texttt{refcoco+\_testA/refexp/refcoco+\_precision\@5} & 86.7 & 88.1 & 86.7 & 87.2 & 86.5 & 86.4 & 86.3 & 86.4 & 87.0 \\
    \texttt{refcoco+\_testB/refexp/refcoco+\_precision\@1} & 46.4 & 47.9 & 46.9 & 48.4 & 47.4 & 48.0 & 47.8 & 47.1 & 47.4 \\
    \texttt{refcoco+\_testB/refexp/refcoco+\_precision\@10} & 90.7 & 92.7 & 91.5 & 92.1 & 89.8 & 91.1 & 91.3 & 90.8 & 92.2 \\
    \texttt{refcoco+\_testB/refexp/refcoco+\_precision\@5} & 84.1 & 85.5 & 83.7 & 85.8 & 83.8 & 84.1 & 85.0 & 84.3 & 85.0 \\
    \texttt{refcoco\_testA/refexp/refcoco\_precision\@1} & 57.4 & 58.8 & 58.4 & 59.1 & 60.2 & 58.6 & 59.0 & 59.0 & 57.8 \\
    \texttt{refcoco\_testA/refexp/refcoco\_precision\@10} & 95.6 & 96.2 & 95.6 & 95.5 & 94.7 & 94.8 & 95.0 & 95.1 & 95.8 \\
    \texttt{refcoco\_testA/refexp/refcoco\_precision\@5} & 91.3 & 91.7 & 86.8 & 91.0 & 90.6 & 90.2 & 90.6 & 91.0 & 91.3 \\
    \texttt{refcoco\_testB/refexp/refcoco\_precision\@1} & 45.0 & 46.8 & 45.4 & 46.8 & 46.4 & 46.8 & 46.8 & 46.5 & 46.1 \\
    \texttt{refcoco\_testB/refexp/refcoco\_precision\@10} & 92.9 & 93.3 & 92.6 & 93.6 & 91.8 & 91.7 & 92.5 & 92.1 & 93.0 \\
    \texttt{refcoco\_testB/refexp/refcoco\_precision\@5} & 86.5 & 87.7 & 86.2 & 87.8 & 86.8 & 85.8 & 87.0 & 87.1 & 87.8 \\
    \texttt{refcocog\_test/refexp/refcocog\_precision\@1} & 59.7 & 62.7 & 61.7 & 62.9 & 59.6 & 59.0 & 59.4 & 58.7 & 59.9 \\
    \texttt{refcocog\_test/refexp/refcocog\_precision\@10} & 96.3 & 97.0 & 96.6 & 97.4 & 96.5 & 96.6 & 96.5 & 96.8 & 96.8 \\
    \texttt{refcocog\_test/refexp/refcocog\_precision\@5} & 92.1 & 93.3 & 92.9 & 93.9 & 92.7 & 92.7 & 92.9 & 93.1 & 93.2 \\
    \texttt{val/refexp/refcoco+\_precision\@1} & 51.6 & 53.5 & 52.5 & 53.1 & 53.3 & 52.6 & 52.7 & 52.1 & 52.7 \\
    \texttt{val/refexp/refcoco+\_precision\@10} & 92.6 & 93.7 & 92.6 & 95.1 & 91.4 & 92.3 & 92.4 & 92.1 & 92.9 \\
    \texttt{val/refexp/refcoco+\_precision\@5} & 86.4 & 88.0 & 86.4 & 89.7 & 86.3 & 86.0 & 86.7 & 86.5 & 86.9 \\
    \texttt{val/refexp/refcoco\_precision\@1} & 50.8 & 53.4 & 52.1 & 53.1 & 53.3 & 52.9 & 52.7 & 52.4 & 52.7 \\
    \texttt{val/refexp/refcoco\_precision\@10} & 94.9 & 95.5 & 95.0 & 95.1 & 93.7 & 94.3 & 94.3 & 94.5 & 94.7 \\
    \texttt{val/refexp/refcoco\_precision\@5} & 89.5 & 90.3 & 89.8 & 89.7 & 89.0 & 89.3 & 89.4 & 89.4 & 89.9 \\
    \texttt{val/refexp/refcocog\_precision\@1} & 60.4 & 62.7 & 60.4 & 62.9 & 59.7 & 59.2 & 59.6 & 58.8 & 60.3 \\
    \texttt{val/refexp/refcocog\_precision\@10} & 96.2 & 97.0 & 96.2 & 97.2 & 96.0 & 96.4 & 96.6 & 96.4 & 96.7 \\
    \texttt{val/refexp/refcocog\_precision\@5} & 92.1 & 93.3 & 92.1 & 93.3 & 92.2 & 92.8 & 92.8 & 93.1 & 92.8 \\
    \textbf{Average} & 76.3 & 77.6 & 76.7 & 77.8 & 69.8 & 69.9 & 70.0 & 69.7 & 70.3 \\
    \bottomrule
    \end{tabular}
  \end{adjustbox}
  \caption{Results for \texttt{grounding\_dino\_swin-t\_pretrain\_zeroshot\_refexp}.}
  \label{tab:grounding_dino_swin_t_pretrain_zeroshot_refexp}
\end{table}

\begin{table}[htbp]
  \centering
  \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{lccccccccc}
    \toprule
    \textbf{Metric} & \textbf{\texttt{O365+GoldG}} & \textbf{\texttt{O365+GoldG+GRIT}} & \textbf{\texttt{O365+GoldG+V3Det}} & \textbf{\texttt{O365+GoldG+GRIT+V3Det}} & \textbf{\texttt{1.3k\_category}} & \textbf{\texttt{1.3k\_and\_40k\_category}} & \textbf{\texttt{1.3k\_and\_40k\_mixup}} & \textbf{\texttt{ovd\_50k\_mixup\_relightening\_4\_21\_open\_finetune}} & \textbf{\texttt{ovd\_50k\_mixup\_relightening\_4\_21\_open\_stage2\_finetune}} \\
    \midrule
    \texttt{ABS/dod/mAP} & 13.4 & 14.5 & 14.5 & 15.9 & 14.1 & 14.8 & 13.1 & 15.2 & 13.3 \\
    \texttt{ABS/dod/mAP\_long} & 14.5 & 16.7 & 16.7 & 17.1 & 14.8 & 13.8 & 13.3 & 15.0 & 11.4 \\
    \texttt{ABS/dod/mAP\_mid} & 13.4 & 13.1 & 13.1 & 22.2 & 14.1 & \textbf{15.5} & 13.2 & 15.7 & 14.2 \\
    \texttt{ABS/dod/mAP\_short} & 13.4 & 14.5 & 14.5 & 15.9 & 13.0 & \textbf{16.3} & 13.4 & 15.4 & 16.0 \\
    \texttt{ABS/dod/mAP\_very\_long} & 11.9 & 13.3 & 13.3 & 14.4 & 14.0 & \textbf{14.2} & 12.5 & 14.5 & 12.8 \\
    \texttt{FULL/dod/mAP} & 15.6 & 17.0 & 16.7 & 17.5 & 15.7 & \textbf{15.8} & 14.3 & 16.5 & 15.2 \\
    \texttt{FULL/dod/mAP\_long} & 16.7 & 18.0 & 18.0 & 18.3 & \textbf{15.1} & 14.7 & 13.6 & 15.4 & 13.2 \\
    \texttt{FULL/dod/mAP\_mid} & 17.3 & 17.7 & 17.7 & 23.4 & 16.2 & 16.4 & 14.5 & 17.1 & 15.7 \\
    \texttt{FULL/dod/mAP\_short} & 15.6 & 17.0 & 16.7 & 17.5 & 17.2 & \textbf{18.0} & 16.7 & 18.8 & 18.7 \\
    \texttt{FULL/dod/mAP\_very\_long} & 13.1 & 15.7 & 15.7 & 13.8 & 13.4 & 13.9 & 12.3 & 14.4 & 13.6 \\
    \texttt{PRES/dod/mAP} & 16.4 & 17.9 & 17.9 & 18.0 & \textbf{16.2} & \textbf{16.2} & 14.7 & 17.0 & 15.8 \\
    \texttt{PRES/dod/mAP\_long} & 17.3 & 18.3 & 18.3 & 18.6 & \textbf{15.2} & 15.1 & 13.7 & 15.5 & 13.9 \\
    \texttt{PRES/dod/mAP\_mid} & 18.4 & 19.0 & 19.0 & 23.7 & \textbf{16.8} & 16.6 & 14.8 & 17.5 & 16.1 \\
    \texttt{PRES/dod/mAP\_short} & 16.4 & 17.9 & 17.9 & 18.0 & \textbf{18.4} & \textbf{18.4} & 17.6 & 19.8 & 19.4 \\
    \texttt{PRES/dod/mAP\_very\_long} & 14.2 & 17.5 & 17.5 & 13.3 & 12.9 & 13.7 & 12.2 & 14.4 & 14.2 \\
    \bottomrule
    \end{tabular}
  \end{adjustbox}
  \caption{Results for \texttt{grounding\_dino\_swin-t\_pretrain\_zeroshot\_concat\_dod}.}
  \label{tab:grounding_dino_swin_t_pretrain_zeroshot_concat_dod}
\end{table}

\begin{table}[htbp]
  \centering
  \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{lccccccccc}
    \toprule
    \textbf{Metric} & \textbf{\texttt{O365+GoldG}} & \textbf{\texttt{O365+GoldG+GRIT}} & \textbf{\texttt{O365+GoldG+V3Det}} & \textbf{\texttt{O365+GoldG+GRIT+V3Det}} & \textbf{\texttt{1.3k\_category}} & \textbf{\texttt{1.3k\_and\_40k\_category}} & \textbf{\texttt{1.3k\_and\_40k\_mixup}} & \textbf{\texttt{ovd\_50k\_mixup\_relightening\_4\_21\_open\_finetune}} & \textbf{\texttt{ovd\_50k\_mixup\_relightening\_4\_21\_open\_stage2\_finetune}} \\
    \midrule
    \texttt{ABS/dod/mAP} & 22.8 & 14.5 & 14.5 & 26.0 & 22.0 & 21.9 & \textbf{23.0} & 22.2 & 22.7 \\
    \texttt{ABS/dod/mAP\_long} & 28.7 & 16.7 & 16.7 & 34.1 & 22.0 & 21.3 & \textbf{22.3} & 22.1 & 22.1 \\
    \texttt{ABS/dod/mAP\_mid} & 22.2 & 13.1 & 13.1 & 30.3 & 28.3 & 28.1 & \textbf{29.5} & 28.7 & 29.5 \\
    \texttt{ABS/dod/mAP\_short} & 22.8 & 14.5 & 14.5 & 26.0 & 22.0 & 21.0 & \textbf{23.7} & 22.1 & 24.5 \\
    \texttt{ABS/dod/mAP\_very\_long} & 14.7 & 13.3 & 13.3 & 14.6 & 13.3 & 14.4 & 14.4 & 13.2 & 12.9 \\
    \texttt{FULL/dod/mAP} & 21.7 & 22.5 & 22.5 & 22.9 & 20.9 & 21.0 & 21.1 & 21.0 & 21.0 \\
    \texttt{FULL/dod/mAP\_long} & 24.0 & 25.1 & 25.1 & 25.4 & 18.7 & \textbf{18.8} & 18.5 & 18.8 & 18.6 \\
    \texttt{FULL/dod/mAP\_mid} & 24.7 & 25.6 & 25.6 & 28.1 & 23.3 & 23.4 & \textbf{23.5} & 23.5 & 23.3 \\
    \texttt{FULL/dod/mAP\_short} & 21.7 & 22.5 & 22.5 & 22.9 & 24.7 & 24.2 & \textbf{25.3} & 24.6 & 25.4 \\
    \texttt{FULL/dod/mAP\_very\_long} & 13.7 & 14.9 & 14.9 & 14.4 & 13.2 & 13.9 & 13.5 & 13.1 & 13.0 \\
    \texttt{PRES/dod/mAP} & 21.3 & 21.5 & 21.5 & 21.9 & 20.5 & 20.6 & 20.4 & 20.5 & 20.4 \\
    \texttt{PRES/dod/mAP\_long} & 22.8 & 23.0 & 23.0 & 23.2 & 17.5 & \textbf{17.9} & 17.1 & 17.7 & 17.4 \\
    \texttt{PRES/dod/mAP\_mid} & 25.5 & 25.2 & 25.2 & 27.4 & 22.1 & \textbf{22.2} & 22.1 & 22.2 & 21.9 \\
    \texttt{PRES/dod/mAP\_short} & 21.3 & 21.5 & 21.5 & 21.9 & 25.5 & 25.1 & \textbf{25.7} & 25.4 & 25.7 \\
    \texttt{PRES/dod/mAP\_very\_long} & 12.9 & 15.0 & 15.0 & 14.2 & 13.1 & \textbf{13.5} & 12.9 & 13.0 & 13.2 \\
    \bottomrule
    \end{tabular}
  \end{adjustbox}
  \caption{Results for \texttt{grounding\_dino\_swin-t\_pretrain\_zeroshot\_parallel\_dod}.}
  \label{tab:grounding_dino_swin_t_pretrain_zeroshot_parallel_dod}
\end{table}

\begin{table}[htbp]
  \centering
  \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{lccccc}
    \toprule
    \textbf{Metric} & \textbf{\texttt{1.3k\_category}} & \textbf{\texttt{1.3k\_and\_40k\_category}} & \textbf{\texttt{1.3k\_and\_40k\_mixup}} & \textbf{\texttt{ovd\_50k\_mixup\_relightening\_4\_21\_open\_finetune}} & \textbf{\texttt{ovd\_50k\_mixup\_relightening\_4\_21\_open\_stage2\_finetune}} \\
    \midrule
    \texttt{data\_time} & 0.7 & 0.7 & 0.8 & 1.7 & 0.8 \\
    \texttt{single\_cat\_ref/avg\_gap} & 34.1 & 33.9 & 37.9 & 37.8 & 38.7 \\
    \texttt{single\_cat\_ref/frac\_positive\_gap} & 86.7 & 86.7 & 89.3 & 88.0 & 90.7 \\
    \texttt{time} & 10.1 & 10.8 & 10.7 & 11.0 & 10.8 \\
    \bottomrule
    \end{tabular}
  \end{adjustbox}
  \caption{Results for \texttt{grounding\_dino\_swin-t\_single\_category\_ref}.}
  \label{tab:grounding_dino_swin_t_single_category_ref}
\end{table}
